Bandit Learning with Positive Externalities

In many platforms, user arrivals exhibit a self-reinforcing behavior: future user arrivals are likely to have preferences similar to users who were satisfied in the past. In other words, arrivals exhibit positive externalities. We study multiarmed bandit (MAB) problems with positive externalities. We show that the self-reinforcing preferences may lead standard benchmark algorithms such as UCB to exhibit linear regret. We develop a new algorithm, Balanced Exploration (BE), which explores arms carefully to avoid suboptimal convergence of arrivals before sufficient evidence is gathered. We also introduce an adaptive variant of BE which successively eliminates suboptimal arms. We analyze their asymptotic regret, and establish optimality by showing that no algorithm can perform better.

==> conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}


Our paper analyzes a benchmark model of a bandit learning problem with positive externalities.  We have several main insights.  First we observe that optimal algorithms for the standard MAB problem such as UCB perform poorly, because they may not find the optimal arm $a^*$ quickly enough.  Second, we show that random exploration also performs poorly, though better than UCB when the externality is relatively weak; again, this is because it spends too much time with the wrong user population.  Finally, we construct a lower bound on the achievable regret, and show that it is tight to leading order in $T$ by developing Balanced-Exploration algorithm which achieves the lower bound by exploring the arms in a structured fashion.  

There are several directions in which we believe our results can be generalized.  First, we believe that the suboptimal performance of UCB will generically hold for {\em any} algorithm that achieves optimal $O(\ln(T))$ regret without the knowledge of time horizon $T$ for the standard stochastic MAB problem (without externalities) (e.g., Thompson sampling), using a similar argument to UCB.  Indeed, an interesting feature of our setting is that we have to obtain sufficiently many samples from suboptimal arms early in our exploration process, since otherwise even the opportunity to learn about these arms may fade away.  Second, we believe our results generalize naturally to rewards with general distributions with bounded support.  Finally, our model uses an extreme model of payoffs: users can only receive positive rewards on preferred arms.  More generally, an interesting open direction is to consider a model with ``smoother'' positive externalities, where future users have higher utility from arms that were successful in the past; e.g., one approach may involve modeling users through covariates that are self-reinforcing.  We leave such a model for future work.

==> extensions.tex <==
% !TEX root = root.tex


\section{Extensions}
\label{sec:extensions}

%\subsection{Regret Scaling with the Number of Arms}
%
%We now to develop a lower bound on regret scaling with respect to both $m$ and $T$ and also show that the performance of BE is optimal. 
%We first obtain the lower-bounds below.
%
%\begin{theorem}\label{thm:LowerBound_m}
%\begin{enumerate}
%\item For $\alpha < 1$, there exists no policy with $ \mathbb E[R_T] = o (m^2 \ln T +  m  T^{1-\alpha} \ln^\alpha T)$ on all sets of Bernoulli reward distributions.
%\item For $\alpha = 1$, there exists no policy with $ \mathbb E[R_T] = o (m^2 \ln T + m \ln^2 T)$ on all sets of Bernoulli reward distributions.
%\item For $\alpha > 1$, there exists no policy with $ \mathbb E[R_T] =  o (m^2 \ln T +  m \ln^\alpha T) $ on all sets of Bernoulli reward distributions.
%\end{enumerate}
%\end{theorem}
%
%
%We now show that the above lower bound is tight by using the Balanced-Exploration($n$) Algorithm as in \ref{sec:waterfill}. 
%
%\begin{theorem}\label{thm:Balanced-Exploration_m}
%Suppose $w_k$, $k = 0, 1, 2, \ldots$, is any sequence such that $w_k \to \infty$ as $k \to \infty$.  Then the regret of the BE algorithm, with $n = w_T( \ln T + \ln m)$ is as follows: 
%\begin{enumerate}
%\item If $0< \alpha < 1$ then $\mathbb E[R_T] = O(w_T( m^2 ( \ln T + \ln m) +  m ( \ln T + \ln m)^\alpha  T^{1-\alpha})).$
%\item If $\alpha = 1$ then $\mathbb E[R_T] = O(w_T(m^2 ( \ln T + \ln m) + m \ln^2 T)).$
%\item If $\alpha >1$ then $\mathbb E[R_T] = O(w_T(m^2 ( \ln T + \ln m) +  m ( \ln T + \ln m)^\alpha)).$
%\end{enumerate}
%\end{theorem}
%




 
%For each $a$ and $k$ we have that $ \frac{X_k}{\lambda_a(k)}$ has mean $\mu_a$, and that $0\le  \frac{X_k}{\lambda_a(k)} \le \lambda_a^{-1}(k) \le c^{-1}$. Consider the following lemma. 

%\begin{lemma}
%$$\P\left( \hat{\mu}_a(t) - \mu_a \ge \epsilon | T_a(t) = k\right) \le \E\left[\exp\left(-2 \frac{ \epsilon^2 k}{c^2}\right)\right],  $$
%and
%$$\P\left(  \mu_a -  \hat{\mu}_a(t) \ge \epsilon \right) \le  \E\left[\exp\left(-2 \frac{ \epsilon^2 k}{c^2}\right)\right] . $$
%\end{lemma}
%\begin{proof}
%We will show the result for the variation of the algorithm where at each time $t$ pull arm $I_t \in \arg\inf_{a \in A(t)} S_a(t-1),$
% with ties broken lexicographically. Thus, the policy is deterministic given the past. The proof for the actual policy is identical but with few further simple steps, as we will explain towards the end. 
% 
% Let $\{\mathcal F_t\}_{t\ge0}$ represent the filtration which captures what is known to the platform at each time $t$. 
%Fix $\lambda>0$. Using Markov Inequality we get
%\begin{align*}
%& \P\left( \hat{\mu}_a(t) - \mu_a \ge \epsilon \right) \\
%		&=  \P\left( \exp(\lambda T_a(t)(\hat{\mu}_a(t) -  \mu_a - \epsilon))\ge 1 \right) \\
%		& =  \P\left(\exp\left(\lambda\sum_{k=1}^{t} \mathbbm{1}(I_k = a) \left( \frac{X_k}{\lambda_a(k)}  - \mu_a -\epsilon\right)\right)\ge 1 \right) \\
%		& \le  \E\left[\exp\left(\lambda\sum_{k=1}^{t} \mathbbm{1}(I_k = a) \left( \frac{X_k}{\lambda_a(k)}  - \mu_a -\epsilon\right)\right) \right] \\
%		& = \E\left[\E\left[\exp\left(\lambda\sum_{k=1}^{t} \mathbbm{1}(I_k = a) \left( \frac{X_k}{\lambda_a(k)}  - \mu_a -\epsilon\right)\right) \Big |\mathcal{F}_{t-1} \right] \right] \text{\virag{$\lambda$  $F_{t}$-measurable for each $t$?}}\\
%		& = \E\left[\exp\left(\lambda\sum_{k=1}^{t-1} \mathbbm{1}(I_k = a) \left( \frac{X_k}{\lambda_a(k)}  - \mu_a -\epsilon\right)\right) \E\left[ \exp\left( \lambda \mathbbm{1}(I_t = a) \left( \frac{X_t}{\lambda_a(t)}  - \mu_a -\epsilon\right) \right) \Big |\mathcal{F}_{t-1} \right] \right]
% \end{align*}
%Here, \virag{use convex dominance via RV bounded by $c^{-1}$ but with same mean}
% \begin{multline*} \E\left[ \exp\left( \lambda \mathbbm{1}(I_t = a) \left( \frac{X_t}{\lambda_a(t)}  - \mu_a -\epsilon\right) \right) \Big |\mathcal{F}_{t-1} \right] \\ = \E\left[  \exp\left(- \lambda\mathbbm{1}(I_t = a)  \epsilon\right) \right] \E\left[ \exp\left(\lambda \mathbbm{1}(I_t = a) \left( \frac{X_t}{\lambda_a(t)}  - \mu_a\right) \right) \Big |\mathcal{F}_{t-1} \right]
% \end{multline*}
% Further, from Hoeffding's Lemma we get 
% $$\E\left[ \exp\left(\lambda \mathbbm{1}(I_t = a) \left( \frac{X_t}{\lambda_a(t)}  - \mu_a\right) \right) \Big |\mathcal{F}_{t-1} \right] \le  \exp\left( \mathbbm{1}(I_k = a) \frac{\lambda^2 }{8(\lambda_a(t))^2}\right) .$$
% Thus, we get
% $$ \P\left( \hat{\mu}_a(t) - \mu_a \ge \epsilon \right) = \E\left[\exp\left(\lambda\sum_{k=1}^{t-1} \mathbbm{1}(I_k = a) \left( \frac{X_k}{\lambda_a(k)}  - \mu_a -\epsilon\right)\right)\exp\left(  \mathbbm{1}(I_t = a)\left( \frac{\lambda^2 }{8(\lambda_a(t))^2} -\lambda \epsilon\right)\right)\right].$$
% Using indnduction, we get
% $$ \P\left( \hat{\mu}_a(t) - \mu_a \ge \epsilon \right) =\E\left[ \exp\left(\sum_{k=1}^{t} \mathbbm{1}(I_k = a) \left(\frac{\lambda^2 }{8(\lambda_a(k))^2} -\lambda\epsilon\right)\right)\right].$$
% 
%
%




%We will prove the result for $\alpha = 1$. The result for general $\alpha$ follows using essentially the same argument. For each $a$ and $k$ we have that $ \frac{X_k}{\lambda_a(k)}$ has mean $\mu_a$, and that $0\le  \frac{X_k}{\lambda_a(k)} \le \lambda_a^{-1}(k)$. Consider the following lemma. 
%
%\begin{lemma}
%$$\P\left( \hat{\mu}_a(t) - \mu_a \ge \epsilon \right) \le \E\left[\exp\left(-\frac{2T_a^2(t) \epsilon^2}{\sum_{k=1}^{t} \lambda_a^{-2}(t)\mathbbm{1}(I_t = a)}\right)\right],  $$
%and
%$$\P\left(  \mu_a -  \hat{\mu}_a(t) \ge \epsilon \right) \le  \E\left[\exp\left(-\frac{2T_a^2(t) \epsilon^2}{\sum_{k=1}^{t} \lambda_a^{-2}(t)\mathbbm{1}(I_t = a)}\right)\right] . $$
%\end{lemma}
%\begin{proof}
%We will show the result for the variation of the algorithm where at each time $t$ pull arm $I_t \in \arg\inf_{a \in A(t)} S_a(t-1),$
% with ties broken lexicographically. Thus, the policy is deterministic given the past. The proof for the actual policy is identical but with few further simple steps, as we will explain towards the end. 
% 
% Let $\{\mathcal F_t\}_{t\ge0}$ represent the filtration which captures what is known to the platform at each time $t$. 
%Fix $\lambda>0$. Using Markov Inequality we get
%\begin{align*}
%& \P\left( \hat{\mu}_a(t) - \mu_a \ge \epsilon \right) \\
%		&=  \P\left( \exp(\lambda T_a(t)(\hat{\mu}_a(t) -  \mu_a - \epsilon))\ge 1 \right) \\
%		& =  \P\left(\exp\left(\lambda\sum_{k=1}^{t} \mathbbm{1}(I_k = a) \left( \frac{X_k}{\lambda_a(k)}  - \mu_a -\epsilon\right)\right)\ge 1 \right) \\
%		& \le  \E\left[\exp\left(\lambda\sum_{k=1}^{t} \mathbbm{1}(I_k = a) \left( \frac{X_k}{\lambda_a(k)}  - \mu_a -\epsilon\right)\right) \right] \\
%		& = \E\left[\E\left[\exp\left(\lambda\sum_{k=1}^{t} \mathbbm{1}(I_k = a) \left( \frac{X_k}{\lambda_a(k)}  - \mu_a -\epsilon\right)\right) \Big |\mathcal{F}_{t-1} \right] \right] \\
%		& = \E\left[\exp\left(\lambda\sum_{k=1}^{t-1} \mathbbm{1}(I_k = a) \left( \frac{X_k}{\lambda_a(k)}  - \mu_a -\epsilon\right)\right) \E\left[ \exp\left( \lambda \mathbbm{1}(I_t = a) \left( \frac{X_t}{\lambda_a(t)}  - \mu_a -\epsilon\right) \right) \Big |\mathcal{F}_{t-1} \right] \right]
% \end{align*}
%Here, 
% \begin{multline*} \E\left[ \exp\left( \lambda \mathbbm{1}(I_t = a) \left( \frac{X_t}{\lambda_a(t)}  - \mu_a -\epsilon\right) \right) \Big |\mathcal{F}_{t-1} \right] \\ = \E\left[  \exp\left(- \lambda\mathbbm{1}(I_t = a)  \epsilon\right) \right] \E\left[ \exp\left(\lambda \mathbbm{1}(I_t = a) \left( \frac{X_t}{\lambda_a(t)}  - \mu_a\right) \right) \Big |\mathcal{F}_{t-1} \right]
% \end{multline*}
% Further, from Hoeffding's Lemma we get 
% $$\E\left[ \exp\left(\lambda \mathbbm{1}(I_t = a) \left( \frac{X_t}{\lambda_a(t)}  - \mu_a\right) \right) \Big |\mathcal{F}_{t-1} \right] \le  \exp\left( \mathbbm{1}(I_k = a) \frac{\lambda^2 }{8(\lambda_a(t))^2}\right) .$$
% Thus, we get
% $$ \P\left( \hat{\mu}_a(t) - \mu_a \ge \epsilon \right) = \E\left[\exp\left(\lambda\sum_{k=1}^{t-1} \mathbbm{1}(I_k = a) \left( \frac{X_k}{\lambda_a(k)}  - \mu_a -\epsilon\right)\right)\exp\left(  \mathbbm{1}(I_t = a)\left( \frac{\lambda^2 }{8(\lambda_a(t))^2} -\lambda \epsilon\right)\right)\right].$$
% Using indnduction, we get
% $$ \P\left( \hat{\mu}_a(t) - \mu_a \ge \epsilon \right) =\E\left[ \exp\left(\sum_{k=1}^{t} \mathbbm{1}(I_k = a) \left(\frac{\lambda^2 }{8(\lambda_a(k))^2} -\lambda\epsilon\right)\right)\right].$$
% 
%Note that the above argument holds even if $\lambda$ is a positive random variable. Thus, we can set 
%\end{proof}
%		&\le \E\left[\exp\left(\lambda\sum_{k=1}^{t-1} \left( \frac{X_k}{\lambda_a(k)} \mathbbm{1}(I_k = a) - \mu_a\right)\right) \E\left[\exp\left( \frac{X_k}{\lambda_a(k)} \mathbbm{1}(I_t = a) - \mu_a\right) \right]\exp(-\lambda T_a(t)\epsilon) \right] 


%
%Using ...proof of Hoeffding's inequality.... we get
%
%Thus, using definition of $l_a(t)$ we get
%
%%\begin{align*}
%%\P\left( u_a(t)  \ge \mu_a + \frac{\delta}{2}) & = \P\left( \hat{\mu}_a(t) + \frac{1}{T_a(t)} \sqrt{  \ln T \sum_{k=1}^{t} \lambda_a^{-2}(t)\mathbbm{1}(I_t = a)} \ge \mu_a + \frac{\delta}{2}\right) \\
%% & \le 
%%\end{align*}
%
%$$\P\left( l_a(t)  \ge \mu_a |  \mathcal{F}_{t-1}\right)  \le \exp ( - 2 \ln T) = T^{-2}.$$
%Similarly, we get
%$$\P\left( u_a(t)  \le \mu_a |  \mathcal{F}_{t-1}\right)  \le \exp ( - 2 \ln T) = T^{-2}.$$
%
%Unconditioning w.r.t. $\mathcal{F}_{t-1}$ we obtain $\P\left( l_a(t)  \ge \mu_a \right)  \le T^{-2}$ and $\P\left( u_a(t)  \le \mu_a \right)  \le T^{-2}$ for each $a$. 



%
%Consider the following lemma.
%
%\begin{lemma}
%There exists a constant $c'$ such that for $t' =c' \ln T$ we have (i) $\P(T_a(t') \le \gamma \ln T, a\in A(t')) \le T^{-2}$, and (ii) $\P(T_{a^*}(t') \le \gamma \ln T) \le 3T^{-2}$. 
%\end{lemma}
%\begin{proof}
%Recall $\Delta > \min_a \mu_a$. Thus, $\P(X_t = 1) \ge c\Delta$ for each $t$ under UCB-LCB algorithm. Thus, using standard Chernoff bound, there exists a constant $c_1$ such that for $t' = c_1 \ln T$ we have 
%$\P(\sum_{t=1}^{t'} X_t \le m \gamma \ln T + m) \le e^{-2 \ln T}$. Since under UCB-LCB algorithm we have $|S_b(t) - S_{b'}(t)| \le 1$ for each $b,b' \in A(t)$, $\P(\exists a \in A(t') \text{s.t.} S_a(t') \le \gamma \ln T ) \le e^{-2 \ln T}$. Thus, $\P(\exists b \in A(t') \text{s.t.} T_b(t') \le \gamma \ln T ) \le e^{-2 \ln T}$. From this the first part of lemma follows, and also that $\P(T_{a^*}(t') \le \gamma \ln T, a^*\in A(t')) \le T^{-2}$. 
%
%The second part of the lemma follows by nothing that
%\begin{align*}
% \P(T_{a^*}(t') \le \gamma \ln T) & = \P(T_{a^*}(t') \le \gamma \ln T, a^*\in A(t')) + \P(T_{a^*}(t') \le \gamma \ln T, a^*\notin A(t')) \\
%  &  \le T^{-2} +  \P(T_{a^*}(t') \le \gamma \ln T, a^*\notin A(t')) \\
%   & \le T^{-2} +  \P( a^*\notin A(t')) \\
%   & \le T^{-2} +  \P(u_{a^*}(t) \le \mu_{a^*}) + \P(l_a(t) \ge \mu_a) \\
%   & \le T^{-2} +T^{-2} +T^{-2}.
% \end{align*}
%\end{proof}
%
%Now, 
%\begin{align*}
%\E[T_a(T)] & \le \E[T_a(T) | a\notin A(t')] + T \P(a\in A(t')) \\
%		& \le t' + T \P(a \in A(t')) \\
%		& = c' \ln T + T \P(a\in A(t'))
%\end{align*}
%
%Thus, we will be done if we show that $\P(a \in A(t'))= O(T^{-2})$. Using union bound and \ref{lemma:deltaBounds}, we obtain that 
%
%\begin{align*}
%\P(a \in A(t')) & \le \P(T_a(t') \le \gamma \ln T, a\in A(t')) + \P(T_{a^*}(t') \le \gamma \ln T, a\in A(t')) \\
%  &  + \P(T_a(t') \ge \gamma \ln T, T_{a^*}(t') \ge \gamma \ln T, a\in A(t')) \\
% & \le T^{-2} + \P(T_{a^*}(t') \le \gamma \ln T) \\& + P(T_a(t') \ge \gamma \ln T, T_{a^*}(t') \ge \gamma \ln T, a\in A(t')) \\
% & \le 4T^{-2} + \P(T_a(t') \ge \gamma \ln T, T_{a^*}(t') \ge \gamma \ln T,  l_{a^*}(t) \le u_a(t)  ) \\
% & \le 4T^{-2} + \P( u_a(t) - l_{a^*}(t) \ge 0 \big| T_a(t') \ge \gamma \ln T, T_{a^*}(t') \ge \gamma \ln T) \\
%\end{align*}
%
%Under $T_a(t') > \gamma \ln T, T_{a^*}(t') \ge \gamma \ln T$, from Lemma~\ref{lemma:deltaBounds} we have $u_a(t) - l_{a*}(t) \le \hat{\mu}_a(t) - \hat{\mu}_{a^*}(t) + \frac{\delta}{8} $. 
%
%Thus, 
%
%\begin{align*}
%&\P( u_a(t) - l_{a^*}(t) \ge 0 \big| T_a(t') \ge \gamma \ln T, T_{a^*}(t') \ge \gamma \ln T) \\
%& \le \P( \hat{\mu}_a(t') - \mu_a \ge \frac{\delta}{8} \big| T_a(t') \ge \gamma \ln T) + \P(\mu_{a^*} - \hat{\mu}(t)_{a^*} \ge \frac{\delta}{8} \big|  T_{a^*}(t') \ge \gamma \ln T)
%\end{align*}
%
%%$u_a(t) \le  \hat{\mu}_a(t) + \frac{\delta}{8}$ and $l_a(t) \ge \hat{\mu}_a(t) - \frac{\delta}{8}$
%
%
%Indeed, using Hoeffding's inequality and Lemma~\ref{lemma:lambda_bound} we obtain
%$$\P\left( \hat{\mu}_a(t) - \mu_a \ge \frac{\delta}{8} \big| T_a(t) = k\right) \le \exp\left(-\frac{2k \delta^2}{64c}\right)$$
%Thus, 
%$$\P\left( \hat{\mu}_a(t) - \mu_a \ge \frac{\delta}{8} \big| T_a(t) \ge k\right) \le \exp\left(-\frac{k \delta^2}{32c}\right)$$
%
%Similarly, 
%$$\P\left(\mu_{a^*} - \hat{\mu}_{a^*}(t) \ge \frac{\delta}{8} \big| T_{a^*}(t') \ge k \right) \le \exp\left(-\frac{k \delta^2}{32c}\right)$$
%
%Using $k = \gamma \ln T$ and definition of $\gamma$ we get
%
%$$\P( u_a(t) - l_{a^*}(t) \ge 0 \big| T_a(t') \ge \gamma \ln T, T_{a^*}(t') \ge \gamma \ln T) \le 2 \exp(-2 \ln T) = 2 T^{-2}.$$
%
%Hence the result follows. 
%%
%% Now, consider $t' = 3 m c \Delta\ln T$. Since $|S_a - S_a'| \le 1$ under UCB-LCB algorithm, we have
%% $$\P(T_a(t') \le c \Delta \ln T) \le \P( S_a(t') \le c \Delta \ln T) \le  \P( \sum_{b\in A} S_a(t') \le 2m c \Delta \ln T)
%% \le \exp(-2mc\Delta \ln T) $$
%%
%%%Recall, $\delta = \min_{a\neq a^*} (\mu_{a^*} - \mu_a)$. Let $\gamma$ be such that $\sqrt{\frac{c}{\gamma}} = \frac{\delta}{8}$. 
%%
%%
%%
%%
%%Now, consider an arm $a \neq a^*$. We show that $E[T_a(T)] = O(\ln T)$. Let $ \kappa \ln T$ where $\kappa = \frac{2 \gamma}{c \min_a \mu_a}$. Then, since probability of 
%%
%%$$ E[T_a(T)] \le T \P(a \in A(t')) + \kappa \ln T.$$ 
%%
%%We bound below $\P(a \in A(t'))$. 
%%
%%Thus, 
%%$$\P(a\in A(t')) \le \P(l_{a^*}(t) \le u_a(t)) $$ 
%%
%%
%


 

%\subsection{Importance of Knowing Time Horizon}
%
%If the time horizon $T$ is not known a priori, then this is not an issue in the standard MAB setting as the algorithms such as UCB and Thompson Sampling ensure optimal performance for each $T$. We show below that this is not possible in presence of positive externalities. In particular we show that the best possible regret achievable if $T$ is set adversarially is almost linear in $T$. 
%
%\begin{theorem}
%Fix constants $\epsilon, C > 0$.
%\begin{enumerate}
%\item For $\alpha < 1$ there exists no policy  such that $\E[R_T] \le C \frac{T}{\ln ^{\alpha+\epsilon} T}$ for each $T$ on all sets of Bernoulli reward distributions. 
%\item For $\alpha = 1$ there exists no policy such that $\E[R_T] \le C \frac{T}{\ln ^{\epsilon} T}$ for each $T$ on all sets of Bernoulli reward distributions. 
%\item For $\alpha > 1$ there exists no policy such that $\E[R_T] \le C \frac{T}{\ln ^{\epsilon} T}$ for each $T$ on all sets of Bernoulli reward distributions. 
%\end{enumerate}
%\end{theorem}
%
%\virag{The powers of $\ln $ may not be accurate yet, but something like this holds.}
%
%
%
%
%
%\subsection{Sticky Users}
%
%Till now, we assumed that if an arm is pulled indefinitely the arrivals which like the other arms get thinned. Now we consider a variant where a fraction $\eta_a$ of the population always like arm $a$ unconditionally. The rest of the population is affected by the externalities.  Here, the probability that an arm is preferred is modified as follows: 
%
%$$\lambda_a(t) = \eta_a + (1 - \eta_a) \frac{f(N_a)}{\sum_b f(N_b)}.$$ 
%
%
%The following theorem provides performance of the \Oracle{} which always pulls arm $a^*$. 
%
%\begin{theorem}\label{thm:Oracle_Sticky}
%Suppose $\alpha>0$. Let $\theta^\alpha = \sum_{a\neq a^*} \theta_a^\alpha$.  The expected cumulative reward $\mathbb E[\Gamma_T^*]$ for the \Oracle{} satisfies:
%\begin{enumerate}
%\item $\displaystyle \mathbb E[\Gamma_T^*]  \le  \mu_{a^*} T - (1-\eta_{a^*})\mu_{a^*}\theta^\alpha\sum_{k=1}^T \frac{1}{(k + \theta_{a^*} - 1)^\alpha + \theta^\alpha}.$
%\item $\displaystyle \mathbb E[\Gamma_T^*] \ge  \mu_{a^*} T - \theta^\alpha \sum_{k=1}^{T} \frac{ 1}{(k+\theta_{a^*})^\alpha + \eta_{a^*} \theta^\alpha}-1 .$
%\end{enumerate}
%\end{theorem}
%
%The proof is similar to that for Theorem~\ref{thm:Oracle}. The lower bound developed in Section~\ref{sec:lower} also easily extends to this setup. Again, it can be shown that the lower bound is tight as follows. We use the idea of Balanced exploration to estimate both $\eta_a$ and $\mu_a$ for each arm $a$. 
%
%For ease of exposure, assume for now that $m=2$ and $A = \{a,b\}$. We first do balanced exploration for $O(\ln T)$ time as defined earlier. This ensures that $\frac{f(N_a)}{\sum_b f(N_b)}$ is close to $\frac{1}{2}$ for each arm. Thus, we can obtain an estimate of $(\eta_{a'} + (1 - \eta_{a'}) \frac{1}{2})\mu_{a'}$ for each arm $a'$. We then do balanced exploration, but pulling arm more often to ensure that approximately $N_a$ twice as much as $N_b$. With this, we can obtain an estimate of $(\eta_{a} + (1 - \eta_{a}) \frac{2}{3})\mu_a$ for arm $a$, and $(\eta_{b} + (1 - \eta_{b}) \frac{1}{3})\mu_b$ for arm $b$. This too takes  $O(\ln T)$ time. Form this estimates of $\eta_a$ and $\mu_a$ can be obtained. 
%
%\subsection{Positive Rewards for Non-preferred Arms}
%
%Till now, if the arm pulled is not preferred by the arrival the reward obtained was $0$. We now generalize this as follows.  The reward obtained when the arm is disliked is Bernoulli($\epsilon$). \virag{this can be much further generalized actually.} Again, the same lower bounds apply and the algorithm of the flavor used for sticky users should work here as well. 
%
%\virag{Above, the argument to externality function is the reward obtained at the arms. Alternatively, we could have the argument to externality function as the rewards obtained by the arrivals of the corresponding classes. Situation here is somewhat trickier. We still believe Balanced exploration achieves optimal performance. May be analyzable via Polya Urn model? Good toy problem to give to a student perhaps.} 
%
%
%


==> introduction.tex <==
% !TEX root = root.tex

\section{Introduction}
\label{sec:intro}

A number of different platforms use multiarmed bandit (MAB) algorithms today to optimize their service: \virag{add citations for each example?} e.g., search engines and information retrieval platforms; e-commerce platforms; and news sites.  In all cases, the basic application of MAB strategies is to adaptively determine the most preferred options (search results, products, news articles, etc.) to maximize rewards.  Optimal algorithms trade off {\em exploration} (acquiring information about lesser known options) against {\em exploitation} (of better known options).

As a result of the use of such policies, the data that these platforms use to make decisions has an inherent sampling bias: the data collection is endogenous to the platform, and not independent from past decisions.  One potential effect that can exacerbate this bias is a shifting user population.  User preferences are often heterogeneous, so future arrivals may be biased towards users who expect to have positive experiences based on the evolution of the platform.

We model the impact of this type of bias by considering a setting in which a platform faces many types of users that can arrive.  Each user type is distinguished by preferring a subset of the item types above all others.  The platform is not aware of either the type of the user, or the item-user payoffs.  Our model is distinguished by the presumption that there are {\em positive externalities} (also called positive network effects) among the users \cite{katz1994systems}: in particular, if one type of item generates positive rewards, users who prefer that type of item become more likely to arrive in the future.  This is a significant effect in real platforms: for example, if a news site generates articles that are liberal (resp., conservative), then it is most likely to attract additional users who are liberal (resp., conservative) \cite{adamic2005political}.  

In some settings, a platform might choose to personalize its services. This strategy is reasonable if the platform is able to obtain fine-grained data on the preferences of each user. This is the theme of much recent work on {\em contextual bandits}; see, e.g., \cite{langford2008epoch, slivkins2011contextual, perchet2013multi} and \cite{Buc12} for a survey of early work.  In such a model, it is important that either (1) enough observable covariates are available to group different users together as decisions are made; or (2) users have long life so that the platform has time to learn about them. But what if the covariates are not very informative about users' preferences, or if the users are short-lived. Further, it is not always possible to personalize services, e.g, when users are anonymous. \virag{any examples of platforms where personalization is just not possible for anybody?}

%There are broadly two ways to maximize reward.  First, the platform might aim for fine-grained data on the preferences of each user, and use this to {\em personalize} the service.  This is the theme of much recent work on {\em contextual bandits}; see, e.g., \cite{langford2008epoch, slivkins2011contextual, perchet2013multi} and \cite{Buc12} for a survey of early work.  In such a model, it is important that either (1) enough observable covariates are available to group different users together as decisions are made; or (2) users are long-lived enough that the platform has time to learn about them.  In this view, the platform essentially knows the user type, and thus can maximize rewards largely independently for each class of users.  But what if these conditions do not hold: in other words, what if context does not provide sufficient information about user type, and users are shorter-lived?

%\rj{One concern I have about this framing: time acts as a capacity constraint in our model, which means that *even* if we have context and users are long-lived, the problem with network effects is different from the problem without network effects...Ultimately I decided that was a second-order point, but let's discuss.}

Our paper quantifies the consequences of positive externalities for bandit learning in a benchmark model where users are short-lived (one interaction per user), and where the platform is unable to observe the user's class on arrival.  As a result, the platform can only use observed rewards to optimize both arm and user type.  In the model we consider, there is a set of $m$ arms. A given arriving user prefers a subset of these arms over the others; in particular, all arms other than the preferred arms generate zero reward. A preferred arm $a$ generates a Bernoulli reward with mean $\mu_a$.  The probability that a user preferring arm $a$ arrives at time $t$ is proportional to $(S_a(t-1) + \theta_a)^\alpha$, where $S_a(t-1)$ is the total reward observed from arm $a$ in the past and $\theta_a$ captures the initial conditions. 

We consider $0 < \alpha < \infty$: when $\alpha$ is near zero, the positive externality is weak; when $\alpha$ is large, the positive externality is strong.  The platform aims to maximize cumulative reward up to time horizon $T$. We study the asymptotic scaling of cumulative regret at $T$ as $T \to \infty$. 

We evaluate our performance by measuring regret against an ``offline'' oracle that knows mean $\mu_a$ for each arm $a$, but does not know the arriving class of each user.  In particular, the oracle we consider always chooses the arm $a^* = \arg \max_a \mu_a$.  Because of the positive externality, this choice causes the user population to shift entirely to users preferring arm $a^*$ over time. Since we assume that $\theta_a$ is fixed and does not scale with $T$, this choice achieves asymptotically optimal performance to leading order in $T$.
%\rj{If the initial conditions are not balanced across all arms and $T$ is small this will not be an optimal oracle...}

At the heart of this learning problem is a central tradeoff.  On one hand, because of the positive externality, the platform operator is able to move the user population towards the profit maximizing population.  On the other hand, because of precisely the same effect, {\em mistakes} are amplified as well: if rewards are generated on suboptimal arms, the positive externality causes more users that prefer those arms to arrive in the future. The design of an optimal algorithm for this problem must balance these two effects: leverage the positive externality to converge to the correct user population, but prevent the positive externality from leading to convergence to the wrong user population.  This trade-off prevails regardless of the strength of the externality. However, the nature of this tradeoff is significantly affected by its strength. We are able to explicitly quantify this tradeoff in our model. 

Our main contributions are as follows:

($i$) We provide a lower bound for the best possible regret scaling which shows a dramatic effect that may result from the tradeoffs implied by the positive externalities. Our lower bound is structurally different than the one known for the standard MAB setting. 

($ii$) We show that if a benchmark algorithm such as UCB, which is optimal for the standard MAB setting, is applied then the regret can be linear in $T$. This is because UCB ``overexploits'' in a way which may quickly shift the user arrivals towards a population preferring a suboptimal arm. As the arrivals of users which prefer the optimal arm become rare the algorithm may not be able to learn the quality of the optimal arm.

($iii$) The deficiency of UCB exposed above emphasizes the need for an algorithm which keeps the population balanced while exploring the arms. Once enough evidence is obtained to ascertain optimality of an arm, only then the exploitation phase should begin, allowing the user population to shift towards preferring that arm. We present an algorithm which has this characteristic, namely Balanced Exploration algorithm. Additionally, we develop the UCB-LCB algorithm which successively eliminates arms from the exploration process when enough evidence is obtained to ascertain their suboptimality, until only one arm remains. We show that both these algorithms are optimal, in that their regret scalings meet the lower bound.   

($iv$) We explore the importance of explicitly balancing user population in the exploration phase. We study an explore-then-exploit strategy where during the exploration phase the arms are chosen at random. The empirically best arm is then exploited in the exploitation phase. We show that its regret scaling is suboptimal even if the length of the exploration phase is chosen carefully. 

%Our main results reveal that positive externalities substantially change the learning problem.  First, we study the regret performance of UCB \cite{ACF02}, a benchmark optimal algorithm for the MAB problem.  We show that regardless of the value of $\alpha$, UCB can have linear regret; fundamentally, this is because it ``overexploits'', and allows the process to converge to the wrong user population.  Second, we consider the regret performance of a policy that chooses arms uniformly at random at each time step up to some fixed time $\tau$, then exploits the empirical best arm until time $T$.  This policy prevents misconvergence, but also does not learn as efficiently as UCB.  It performs better than UCB for smaller values of $\alpha$, but with performance worsening to linear regret for $\alpha > 1$: when the positive externality is sufficiently strong, the random policy is punished for its unstructured approach to exploration.
%
%Motivated by the observations, we develop a lower bound to the achievable regret, which is structurally quite different than the performance of UCB and random-explore-then-exploit policy. We also develop an new policy that tries to optimally balance the learning and the shifting population dynamics introduced by the positive externality.  This policy also follows an explore-then-exploit structure, like the random policy.  However, during the exploration phase the policy is cautious: it explores the arm with the {\em least} accrued reward, to ensure that the algorithm can observe whether low rewards were simply a consequence of bad luck.  We show that this policy achieves $O(T^{1-\alpha} \ln^\alpha T)$ regret when $0 < \alpha < 1$, $O(\ln^2 T)$ regret when $\alpha = 1$, and $O(\ln^\alpha T)$ regret when $\alpha > 1$.  Further we provide matching lower bounds, showing that this policy is order optimal.  It exploits strong positive externalities when available, but also substantially reduces the probability of exploiting with the wrong user population.  Our results are summarized in Table \ref{tbl:performance}.

\begin{table*}
\begin{center}
\begin{tabular}{c||c|c|c|c|}
 & $\alpha = 0$ & $0< \alpha<1$ & $\alpha = 1$ & $\alpha >1$ \\ 
 \hhline{=#=|=|=|=|}
UCB  		& $O(\ln T)$    	& $\Omega(T)$ 				& $\Omega(T)$	 &	$\Omega(T)$\\
\hline
Random 		& $O(\ln T)$	& $\Omega\left(T^{1-\alpha} \ln ^{\frac{\alpha}{1-\alpha}} T\right)$ & $\Omega\left(T^{\frac{\mu_b}{\mu_b+\theta_{a^*}\mu_{a^*}}}\right)$  & $\Omega(T)$ \\
\hline
Balanced-Exploration 	& $O(\ln T)$	&  $O(T^{1-\alpha} \ln^{\alpha} T)$ 			& $O(\ln^2 T)$	&  $O(\ln^\alpha T)$\\
\hline
Lower Bound	& $\Omega(\ln T)$ 	&  $\Omega(T^{1-\alpha} \ln^\alpha T)$	& $\Omega(\ln^2 T)$  & $\Omega(\ln^\alpha T)$ \\
\hline
\end{tabular}
\end{center}
\caption{\virag{change the order once structure is finalized} Performance comparison of various strategies for different values of $\alpha$. Here, $b = \arg \max_{a\neq a^*} \mu_a$. For Random Explore-then-Exploit policy we assume that $\theta_a$ for each arm $a$ is a positive integer.  %For performance of Random policy subject to $0<\alpha \le 1$, we assume that initial conditions are symmetric across arms, i.e., $\theta_a =1$ for each $a \in A$. 
\label{tbl:performance}
}
\end{table*}


The presence of positive externalities presents a unique technical challenge: since the type of the arriving user determines the preferred arm, the rewards obtained at an arm are no longer i.i.d. They are influenced by the past rewards. Analyzing performance of an algorithm requires characterizing this dependence, which is a challenge. To analyze our UCB-LCB optimal algorithm we model the influence of past via a discrete time martingale and use Freedman's inequality \cite{fre75} to obtain concentration bounds for non-i.i.d.\ rewards. For Random explore-then-exploit algorithm we develop our analysis by viewing the cumulative rewards at each arm as a generalized urn process.   Following classical results in the literature on urn models, we embed this process in a continuous-time branching process, and leverage the resulting representation to characterize performance.

Our work provides a first step towards understanding the influence of positive externalities on bandit learning.  As noted above, our work investigates a setting with different constraints and tradeoffs from much of the existing work on personalization.  Of course, the reality of many platforms is somewhere in between: some user information may be available, though imperfect.  Nevertheless, our work suggests that there are significant consequences to learning when the user population itself can change over time, an insight that we expect to be robust across a wide range of settings.

\subsection{Discussion}
\virag{perhaps should go towards the end of the paper.}

Our contributions expose important qualitative differences relative to conventional MAB strategies, so it is important to discuss our framework vis-\`{a}-vis our goal; namely, expose the types of tradeoffs that positive externalities bring up in MAB learning problems. \virag{too defensive?} We discuss below the assumptions made in our model, ways to relax some of them, and possible future extensions. 

{\em Knowledge of $T$:} One of the benefits of UCB algorithm in standard MAB framework is that it does not assume that time horizon $T$ is known. Our framework is motivated by platforms which are in their initial or middle phase of their growth period with a specific deadline relatively far in the future dictated by its exit strategy or long term goals. In this context assuming that the time horizon $T$ is known is, we believe, a reasonable assumption. 

{\em General reward distribution:} As one may anticipate, our assumption of reward distribution being Bernoulli is not critical. We are able to generalize our results to arbitrary positive reward distributions with bounded support. See appendix for a discussion on this. 

{\em Capacity constraint:} We assume a stream of arrivals with one arrival per unit time for a fixed time horizon $T$. This imposes an implicit constraint on the capacity of the platform. This issue could be resolved by considering a continuous time framework in which arrivals are Poisson-type. 
%The intensity of the arrivals at time $t$ of users who prefer arm $a$ is proportional to $(S_a(t_-) + \theta_a)^\alpha$ where $S_a(t_-) = \lim_{h\to 0^-} (S_a(t - h))$. 
Although the results may look structurally different we believe that the fundamental insights would be similar to those conveyed by our results. 

{\em Scaling w.r.t.\ the number of arms:} We are able to generalize our regret lower bounds to provide scaling laws w.r.t.\ both $m$ and $T$, and show that our Balanced Exploration and UCB-LCB algorithms are near-optimal in regret scaling with a $\log m$ gap from the lower bound. See appendix for a discussion on this. 

{\em Other externality models:} There are several other extensions that might be considered. For example, the effect of negative externalities, wherein dissatisfied users create negative shifts in the preferences of the future user arrivals; memory of the externality, wherein customers may forget the effect of the past evolution; persistent arrivals, wherein a fraction of arrivals are unaffected by the externalities, etc. All these extensions are interesting and within reach, but we decided to focus on the presented model for focus and clarity. 




\subsection{Organization}

The remainder of the paper is organized as follows.  In Section \ref{sec:problem}, we introduce the model, and in Section \ref{sec:oracle} we introduce the oracle benchmark we compare against, and our definition of regret.  In Section \ref{sec:ucb}, we study the suboptimality of the UCB algorithm.  In Section \ref{sec:random}, we study the performance of an algorithm that randomly explores arms before exploiting. Finally, in Section \ref{sec:OptimalRegret}, we prove lower bounds on the performance of any algorithm and show that they are tight by developing an algorithm which achieves them. 
Proofs are provided in the Appendix.
%We conclude in Section \ref{sec:conclusion}.  Omitted proofs can be found in the Appendix.

%% Platforms serving dynamically arriving users make real-time servicing/matching decisions using models developed from data collected in the past. These models suffer from sampling bias as the data collection process is endogenous to the platform and is thus not independent of its past decisions. A prominent source of such bias is shifting user population. User preferences are often heterogeneous and the arrival of users is influenced by the user's perception of the platform with regards to meeting these preferences. 

%% The process of influencing user arrivals may be exogenous to the platform, as in network effects: users in a social group are likely to join the platform if some of its members are already in the platform and are happy with it. It may also be endogenous: online product reviews may reflect preferences of the satisfied and dissatisfied users which may influence future arrivals. In either case, we are interested in self-reinforcing population shifts wherein servicing decisions benefiting population of a given preferences would increase the population with those preferences. Our goal is to study the impact of such a phenomenon on learning, develop insights, and provide learning algorithms in its presence. 

\section{Related Work}

As noted above, our work incorporates the notion of positive externalities, also known as positive network effects or positive network externalities.  (Note that the phrase ``network'' is often used here, even when the externality may not be due to network connection between the users per se.)  See \cite{katz1994systems}, as well as \cite{shy2011short, shapiro1998information} for background.  Positive externalities are extensively discussed in most standard textbooks on microeconomic theory; see, e.g., Chapter 11 of \cite{mas1995microeconomic}.

It is well accepted that online search and recommendation engines produce feedback loops that can lead to self-reinforcement of popular items \cite{anderson2004long, barabasi1999emergence, ratkiewicz2010characterizing, chakrabarti2005influence}.  Our model captures this phenomenon by employing a self-reinforcing arrival process, inspired by classical urn processes \cite{AtK68, Jan04}.

We note that the kind of self-reinforcing behavior observed in our model may be reminiscent of ``herding'' behavior in Bayesian social learning \cite{bikhchandani1992theory, SmS00, ADL11}.  In these models, arriving Bayesian rational users take actions based on their own private information, and the outcomes experienced by past users; under some circumstances, it can be shown that the users will ``herd'', in the sense that after some finite time they all choose the same action.  The central question in that literature is whether individuals act on their own private information or not, rather than following the crowd; indeed, users who herd exhibit a {\em negative} externality on others, as their private information is not shared.  By contrast, in our model users do not have private information; instead, it is the platform that is trying to learn from preferences of users, and users exert {\em positive} externalities on each other.


 
%% We consider a bandit learning model with finite distinct arms and dynamically arriving users with heterogeneous and unknown preferences. We view pulling of each arm as an option presented to a new user. An arm pulled produces a positive reward only if the user has a preference for that arm, otherwise zero reward is obtained. Motivated by the Polya Urn model to capture self-reinforcing property, each new user has a preference for an arm with probability which is proportional to the total reward achieved by the user of that type in the past. 

%% In such a setting we show that the standard UCB learning algorithm which does not account for shifting user population fails poorly. We also study a natural algorithm where each arm is chosen uniformly at random, and demonstrate that this too performs poorly. We also develop an algorithm which obtains significantly lower regret as compared to UCB and Random. We develop an explicit lower-bound for regret under our model and show that our algorithm is asymptotically optimal in that its regret is of the same order as the lower bound. 



==> model.tex <==
% !TEX root = root.tex

\section{Problem Formulation}
\label{sec:problem}

Let $A = \{a_1,a_2,\ldots,a_m\}$ be the set of arms available. %Each arm $a\in A$ is associated with a $[0,1]$ (....do we need this?....) valued distribution $F_a$ with mean $\mu_a$. 
During each time $t \in \{1, \ldots, \infty\}$ a new user arrives, and an arm is ``pulled''; we denote the arm pulled at time $t$ by $I_t$.  We view pulling an arm as presenting the corresponding option to the newly arrived user. Each arriving user prefers a subset of the arms, denoted by $J_t$. We assume that $J_t$ is not known. If arm $a$ is pulled at time $t$ {\em and} if the user at time $t$ prefers arm $a \in A$, then the reward obtained at time $t$ is an independent Bernoulli random variable with mean $\mu_a$, where $\mu_a > 0$ for each $a \in A$. 
%We will call $F_a$ as reward distribution for arm $a$. 
If the user at time $t$ does not prefer the arm pulled then the reward obtained at time $t$ is zero. Let $X_t$ denote the reward obtained at time $t$.

 Let $T_a(t)$ represent the number of times arm $a$ is pulled by time $t$, and $S_a(t)$ represent the total reward accrued by pulling arm $a$ up to time $t$.  Thus $T_a(t) = |\{ s \leq t : I_s = a\}|$, and $S_a(t) = |\{ s \leq t : I_s = a, X_s = 1\}|$.   Let
$$a^* = \arg \max_{a} \mu_{a}.$$
For simplicity, we assume that $a^*$ is unique. We also assume that there exist positive constants $\delta $ and $ \Delta $ such that $\mu_{a^*} - \mu_a > \delta$ for each $a \neq a^*$ and $ \mu_a > \Delta$ for each $a \in A$.  
% \virag{Justify $\Delta$. Reviewer might complain that waterfilling works only when $\Delta>0$. Or relax the assumption...just throw away an arm for which, after repeated failures, you are certain that it is less than some small $\Delta$.}

Suppose there are fixed constants $\theta_a, a \in A$ that denote the initial ``popularity'' of arm $a$.  Define:
\[ N_a(t) = S_a(t) + \theta_a,\ \ \ a \in A. \]
By definition, $N_a(0) = \theta_a$.  We assume that the $t\kth $ user prefers arm $a$ (i.e., $a \in J_t$) with probability $\lambda_a(t)$ independently of other arms, where:
\[ \lambda_a(t) \coloneqq \frac{f(N_a(t-1))}{\sum_{a'} f(N_{a'}(t-1))} \]
for an increasing function $f$. We refer to $f$ as the {\em externality function}. We are primarily interested in the following class of externality functions: 
$$f(x) = x^\alpha,   \quad 0<\alpha <\infty.$$
Intuitively, the idea is that agents who prefer arm $a$ are more likely to arrive if arm $a$ has been successful in the past.  This is a positive externality: users who prefer arm $a$ are more likely to generate rewards when arm $a$ is pulled, and this will in turn increase the likelihood an arrival preferring arm $a$ comes in the future.  The parameter $\alpha$ controls the strength of this externality: the positive externality is stronger when $\alpha$ is larger.

If $f$ is linear ($\alpha = 1$), then we can interpret our model in terms of an urn process.
%\[ \lambda_a(t) = \frac{N_a(t-1)}{\sum_{a'} N_{a'}(t-1)}$
 %We assume that $\lambda_a(1) = \frac{\theta_a}{\sum_{a'} \theta_{a'}}$ where $\theta_a$ are arbitrary positive integers. 
In this view, $\theta_a$ resembles the initial number of balls of color $a$ in the urn at time $t=1$ and $N_a(t)$ resembles the total number of balls of color $a$ added into the urn after $t$ draws. Thus, the probability the $t\kth$ draw is of color $a$ is proportional to $N_a(t)$. In contrast to the standard urn model, in our model we have additional control: namely, we can pull an arm, and thus govern the probability with which a new ball of same color is added into the urn. 

%\virag{Also add the case where each user prefers only one arm. Not so surprisingly, results are similar for both preference models under UCB, Random, and waterfilling policies....Explain why.}

%More generally, we let  

The goal is to choose $I_t$ to maximize the expected total reward accrued in a time horizon $T$.  We let $\Gamma_T$ denote the total reward obtained up to time $T$:
\begin{equation}
\label{eq:reward}
\Gamma_T =  \sum_{t = 1}^T X_t.
\end{equation}

%When a new user arrives an arm is pulled. Let $C = \{c_1,c_2,\ldots,c_n\}$ be the set of user types. If arm $a\in A$ is pulled upon arrival of a user of type $c \in C$ then the reward accrued is Bernoulli($\mu_{ac})$ distributed. Let $R = [\mu_{ac}]_{A\times C}$ be the expected reward matrix. 
%
%Users arrive sequentially. The $t\kth$ arrival is of type $c$ with probability $\lambda_c(t)$. We assume that $\lambda_c(0) = \frac{\theta_c}{\sum_{c'} \theta_{c'}}$ where $\theta_c$ are arbitrary positive constants. For each $t\ge1$ we have $\lambda_c(t) = \frac{N_c(t-1)}{\sum_{c'} N_{c'}(t-1)}$, where $N_c(t)$ for each $c$ is the total reward accrued till time $t$ plus $\theta_c$. In the view of the urn model, $\theta_c$ resembles the initial number of balls of color $c$ in the urn at time $t=0$ and $N_c(t)$ resembles the total number of balls of color $c$ added into the urn after $t$ draws. Thus, the probability with the $t\kth$ draw is of color $c$ is proportional to $N_c(t)$. In contrast to the standard urn model, we introduce a control, namely pulling an arm, which governs the probability with which a new ball of same color is added into the urn. 


\section{Oracle and Regret}
\label{sec:oracle}

%We consider two notions of Oracles. (Should we pick one? Or keep both and give them better names?)
% 
%1.) Oracle 1: Consider an Oracle which knows all system parameters, namely $\mu_a$ for each $a \in A$, $\theta_a$ for each $a\in A$, and function $f$. Further suppose that the time horizon $T$ is known. Then, the optimal policy can be obtained by solving an MDP \virag{Lay out the value iteration explicitly}. We can compute cumulative regret for a policy against expected rewards accrued by such an Oracle based policy.
 
We consider the following \Oracle{} policy as our benchmark.

\begin{definition}[\Oracle{}] 
The $\Oracle$ algorithm  knows the optimal arm $a^*$ and pulls it at all times $t = 1, 2, \ldots$.
\end{definition}

Let $\Gamma_T^*$ denote the reward of this \Oracle{}.  We measure regret against the oracle: given any policy, define $R_T$ as:
\begin{equation}
\label{eq:regret}
 R_T = \Gamma_T^* - \Gamma_T.
\end{equation}
Our goal is to design algorithms that minimize the expected regret $\E[R_T]$.  In particular we focus on characterizing regret performance asymptotically to leading order in $T$, for different values of the externality exponent $\alpha$.  Note that \Oracle{} may not be optimal for finite fixed $T$; however, we show that it is asymptotically optimal as $T \to \infty$.

Unlike in the standard stochastic MAB problem, the expected cumulative reward $\mathbb E[\Gamma_T^*]$ is not $\mu_{a^*} T$, as several arrivals may not prefer the optimal arm. Below, we provide tight bounds on $\mathbb E[\Gamma_T^*]$. For proof see Appendix. 

%Let for each $k\in \mathbb Z_+$ and $0 <\alpha < \infty$, let $H_{n,\alpha} $ be the $n\kth$ harmonic number of power $\alpha$, i.e.,
%
%$$H_{n,\alpha} = \sum_{k=1}^{n} \frac{1}{k^\alpha}.$$
%
%The following properties hold for generalized harmonic functions. 
%
%$$H_{n,\alpha} = 
%\begin{cases}
% O(n^{1-\alpha}), \quad &0<\alpha<1 \\
% O(\ln n), \quad &\alpha = 1 \\
% O(1), \quad &\alpha > 1
% \end{cases}.
% $$
% 
% The following result holds. 

\begin{theorem}\label{thm:Oracle}

Suppose $\alpha>0$. Let $\theta^\alpha = \sum_{a\neq a^*} \theta_a^\alpha$.  The expected cumulative reward $\mathbb E[\Gamma_T^*]$ for the \Oracle{} satisfies:
%\begin{multline*}
%\mu_{a^*} T -  \theta_b^\alpha \left( H_{\ceil{T+\theta_a},\alpha} -  H_{\floor{\theta_a},\alpha}\right)  \le  \mathbb E[\Gamma^*] \\ \le \mu_{a^*} T   -  \mu_a^{1-\alpha} \theta_b^\alpha \left(H_{\floor{T+\theta_b\mu_a^{-\alpha}, \alpha}} - H_{\ceil{\theta_b\mu_a^{-\alpha}, \alpha}} \right) 
%\end{multline*}
%\begin{enumerate}
%\item  
\begin{enumerate}
\item $\displaystyle \mathbb E[\Gamma_T^*]  \le  \mu_{a^*}T - \mu_{a^*}\theta^\alpha\sum_{k=1}^T \frac{1}{(k + \theta_{a^*} - 1)^\alpha + \theta^\alpha}.$
%$\displaystyle \mathbb E[\Gamma^*] \ge \mu_{a^*} T -  \theta^\alpha \left( H_{T+\theta_{a^*},\alpha} -  H_{\theta_{a^*},\alpha}\right) -1 .$
%\item 
\item $\displaystyle \mathbb E[\Gamma_T^*] \ge  \mu_{a^*} T - \theta^\alpha \sum_{k=1}^{T} \frac{ 1}{(k+\theta_{a^*})^\alpha}-1 .$
%$\displaystyle \! \mathbb E[\Gamma^*]  \le  \mu_{a^*} T  -  \mu_{a^*}^{1-\alpha} \theta^\alpha \!\left( \!H_{\floor{\!T+\theta\mu_{a^*}^{-\alpha}\!}, \alpha} \!\!-  H_{\ceil{\theta\mu_{a^*}^{-\alpha}}, \alpha} \! \right) \!\!.$
\end{enumerate}
\end{theorem}

\begin{corollary}\label{cor:Oracle}
We have:
$$\displaystyle \mathbb E[\Gamma_T^*] = 
\begin{cases} 
 \mu_{a^*}T -  \Theta(T^{1-\alpha}), \quad &0<\alpha<1 \\
  \mu_{a^*}T -  \Theta(\ln T), \quad &\alpha = 1 \\
  \mu_{a^*}T - \Theta(1), \quad &\alpha > 1
\end{cases}
$$
\end{corollary}

Note that in all cases, the reward asymptotically is of order $\mu_{a^*} T$.  This is the best achievable performance to leading order in $T$, showing the oracle is asymptotically optimal.

%To check that $\sum_{k=1}^T \frac{1}{(\mu_{a^*} k)^\alpha + \theta^\alpha} = \Omega(T^{1-\alpha})$, note that $\int_1^T \frac{1}{ x^\alpha +c} dx = \int_1^T \frac{x^\alpha - c}{ x^{2\alpha} -c^2} \ge \int_1^T \frac{x^\alpha - c}{ x^{2\alpha} }.$ Then integrate.  

%\begin{proof}
%
%\end{proof}
%Suppose $\theta_a = 1$, with larger $\theta_a$ the rewards only get better.  For simplicity, we will first consider the case where $A=\{a,b\}$, and $a^* = a$. 
%We will study the process $N = \left(N_a(t),N_b(t)\right)_{t\in \mathbb Z_+}$ by analyzing a multitype continuous time Markov branching process $Z = \left(Z_a(\tau), Z_b(\tau)\right)_{\tau \in \mathbb R_+}$ such that its embedded Markov chain, i.e., the discrete time Markov chain corresponding to the state of the branching process at its jump times, is statistically identical to $N$. By jump time we mean the times at which a particle dies; upon death it may give birth to just one new particle, in which case, the size of the process may not change at the jump times. 
%
%We construct $Z$ as follows. Both $Z_a$ and $Z_b$ are themselves independently evolving single dimensional branching processes. Initially, $Z_a$ and  $Z_b$ have one particle each, i.e., $Z_a(0) =\theta_a$ and  $Z_b(0) = \theta_b$. Each particle in $Z_a$ dies at a rate $1$. At the end of its lifetime, the particle belonging to $Z_a$ dies and gives birth to one new particle with probability $1 - \mu_a$ and two new particles with probability $\mu_a$. At time $\tau$, each particle in $Z_b$ dies at the rate $\frac{|Z_a(\tau)|}{f(|Z_a(\tau)|} f(|Z_b(\tau)|)$, and upon death it gives rise to exactly one new particle. Note that $|Z_b(\tau)| = \theta_b$ for all $\tau$. However, jump points in $Z_b$ will be useful.  
%
%We can see that the embedded Markov chain of $Z$ is statistically identical to $N$ as follows. Let $\tau_1, \tau_2, \ldots , \tau_t, \ldots$ represent the jump times of $Z$. Clearly, $Z(\tau_1)$ and $N(1)$ are identically distributed. Further, after the $t\kth$ jump of $Z$, the rate at which $Z_a$ increments is $f(Z_a(\tau_t))$. Thus, the probability that the $(t+1)\kth$ jump of $Z$ belongs to $Z_a$ is $\frac{f(Z_a(\tau_t))}{f(Z_a(\tau_t)) + f(Z_b(\tau_t))}$. This is simulating the preference selection of the $(t+1)\kth$ user arrival. Further, the birth of new particles simulates the selection of optimal matching arm at all times and generation of the positive reward. 
%
%$|Z_a(\tau)|$ is the Yule Process~\cite{..} and is known to have distribution $Geometric(e^{-\mu_a\tau})$ at time $\tau$.  Further, let $P(\tau)$ represent the number of jumps in $Z_b(\tau)$ till time $\tau$. Then, $(P(\tau))_{\tau \in \mathbb R_+}$ is a inhomogeneous Poisson point process with rate $\frac{|Z_a(\tau)|}{f(|Z_a(\tau)|)} \theta_b$. 
%
%Clearly, for each $\tau$ we have
%$$\mathbb P(|Z_a(\tau)| \ge T) \le  (1- e^{-\mu_a\tau})^{T}.$$ 
%%%Put \tau = 3\log T/\mu_b to get small prob.  
%
%By letting $\tau = 3 \mu_a^{-1} \ln T$ we get
%$$\mathbb P(|Z_a(3 \mu_a^{-1} \ln T)| \ge T) \le (1-\frac{1}{T^3})^T \le e^{-\frac{1}{T^2}} = 1 - O(\frac{1}{T^2}).$$
%
%Thus, w.h.p., number of points in $Z$ before time $\tau$ is greater than the time horizon $T$. 
%
%Let $B$ be the total number of arrivals within the time horizon which preferred arm $b$. 
%
%
%Suppose $f(x) = x$. Then,
%
%\begin{align*}
%\mathbb \mathbb E[B] &  \le \mathbb P(|Z_a(3 \mu_a^{-1} \ln T)| \le T) 
%\\ & + \mathbb E\big[P(3 \mu_a^{-1} \ln T) \big| |Z_a(3 \mu_a^{-1} \ln T)| \ge T\big] \\
%& = o(1) + 3 \frac{\theta_b}{\mu_a} \ln T
% \end{align*}
%
%If $f(x) = x^\alpha$ for some $\alpha<1$, then, again we have
%\begin{multline}
%\mathbb E[B] \le T \; \mathbb P(|Z_a(3 \mu_a^{-1} \ln T)| \le T) \\ + \mathbb E\big[P(3 \mu_a^{-1} \ln T) \big| |Z_a(3 \mu_a^{-1} \ln T)| \ge T\big] .
%\end{multline}
% 
%We have $ \mathbb E\big[P(3 \mu_a^{-1} \ln T) \big| |Z_a(3 \mu_a^{-1} \ln T)| \ge T\big] \le \mathbb E\big[P(3 \mu_a^{-1} \ln T)\big]$.....\virag{do we have this?} 
%
%Thus, 
%\begin{align*}
%\mathbb E[B] &\le o(1) + \mathbb E\big[P(3 \mu_a^{-1} \ln T) \big] \\ &= o(1) +  \mathbb E\big[ \int_{\tau=0}^{3 \mu_a^{-1} \ln T} \frac{|Z_a(\tau)|}{f(|Z_a(\tau)|} f(\theta_b) d\tau \big]. 
%\end{align*}
%
%\virag{do we have the last inequality? Integration of rates till time t is mean of Poisson process at t when time-varying rates are deterministic. But that should be okay no?}
%
%Thus, if $f(x) = x^\alpha$ then we have,
%
%If $0<\alpha<1$ then
%\begin{align*}
%\mathbb E[B] &\le o(1) +  \theta_b \mathbb \int_{\tau=0}^{3 \mu_a^{-1} \ln T} E\big[  |Z_a(\tau)|^{1-\alpha}  \big] d\tau \\
%	&\le  o(1) +  \theta_b \mathbb \int_{\tau=0}^{3 \mu_a^{-1} \ln T} E\big[  |Z_a(\tau)|\big]^{1-\alpha}   d\tau \\
%	&=  o(1) +  \theta_b \mathbb \int_{\tau=0}^{3 \mu_a^{-1} \ln T} e^{(1-\alpha)\mu_a \tau}   d\tau \\
%	& = o(1) +  \frac{\theta_b}{(1-\alpha) \mu_a} \Big[  e^{(1-\alpha)\mu_a \tau}  \Big]_0^{3 \mu_a^{-1} \ln T} \\
%	& = 1 +\frac{\theta_b}{(1-\alpha) \mu_a} T^{3(1-\alpha)}
%\end{align*}
%
%\end{proof}













==> optimalregret.tex <==
% !TEX root = root.tex

\section{Optimal Regret}\label{sec:OptimalRegret}
In this section we obtain a lower bound on regret achievable by any policy for each $\alpha$, and show that the lower bounds are tight by developing a policy which achieves this lower bound. 

\subsection{Lower Bounds}
\label{sec:lower}

%In this section, we provide lower bounds that show that to leading order in $T$, the performance of the Balanced-Exploration policy described in the preceding section is essentially optimal.  
To understand our construction of the lower bound, consider the case where the externality function is linear ($\alpha = 1$); the other cases follow similar logic.

Our basic idea is that in order to determine the best arm, any optimal algorithm will need to explore all arms at least $\ln T$ times.  However, this means that after $t' = \Theta(\ln T)$ time, the total reward on any suboptimal arms will be of order $\sum_{b \neq a^*} N_b(t') = \Theta(\ln T)$.  Because of the effect of the positive externality, any algorithm will then need to ``recover'' from having accumulated rewards on these suboptimal arms; we show that even if the optimal arm $a^*$ is pulled from time $t'$ onwards, a regret $\ln^2 T$ is incurred simply because arrivals who do not prefer arm $a^*$ continue to arrive in sufficient numbers. 

\begin{theorem}\label{thm:LowerBound}
\begin{enumerate}
\item For $\alpha < 1$, there exists no policy with $ \mathbb E[R_T] = o (T^{1-\alpha}\ln^{\alpha} T)$ on all sets of Bernoulli reward distributions.
\item For $\alpha = 1$, there exists no policy with $ \mathbb E[R_T] = o (\ln^2 T)$ on all sets of Bernoulli reward distributions.
\item For $\alpha > 1$, there exists no policy with $ \mathbb E[R_T] = o (\ln^\alpha T)$ on all sets of Bernoulli reward distributions.
\end{enumerate}
%1.) Suppose $\alpha \le 1$. Consider a policy which achieves $o(T^{1-\alpha +\epsilon})$ regret for any set of Bernoulli reward distributions. Then, for any set of Bernoulli reward distributions the following holds:
%$$ \mathbb E[R] = \Omega (T^{1-\alpha}\ln^{\alpha} T).$$ 
%2.) Suppose $\alpha = 1$. Consider a policy which achieves $o(T^\epsilon)$ regret for any set of Bernoulli reward distributions. Then, for any set of Bernoulli reward distributions the following holds:
%$$ \mathbb E[R] = \Omega (\ln^2 T).$$
%3.)  Suppose $\alpha \ge 1$. Consider a policy which achieves $o(T^\epsilon)$ regret for any set of Bernoulli reward distributions. Then, for any set of Bernoulli reward distributions the following holds:
%$$ \mathbb E[R] = \Omega (\ln^\alpha T).$$
\end{theorem}



%Let $c_2 = K(\mu_b,\mu'_b) - K(\epsilon,\mu_b) + K(\epsilon,\mu'_b) $. Then, we have 
%$$\mathbb P(e^{-\hat K_{t'}(\mu_b,\mu_b')} \le e^{- c_2 \ln T}) \le  e^{-\epsilon \mu_b t'} \le .$$
%
%Then, 
%
%\begin{align*}
%\mathbb E[ \mathbbm 1(E_3) e^{-\hat K_{t'}(\mu_b,\mu_b')}]  & \ge  T^{-c_2} \mathbb E[\mathbbm 1(E_3) \mathbbm 1(e^{-\hat K_{t'}(\mu_b,\mu_b')} > e^{- c_2 \ln T})] \\
%			&  \ge T^{-c_2} (1 - P(E_3^c) - \mathbb P(e^{-\hat K_{t'}(\mu_b,\mu_b')} \le e^{- c_2 \ln T})) \\
%			& \ge O(T^{-c_2})
%\end{align*}
%
%Thus, $\mathbb P'(E_3) = O(T^{-c_2})$. Further, conditioned on $E_3$ the expected regret incurred under the modified setting is $\Omega(T^\gamma)$ since arm $b$ is optimal in this setting. Thus, by choosing $\gamma > c_2$, expected overall regret incurred under modified setting is $\Omega(T^{\gamma - c_2})$ which is $\omega(\log^2 T)$, hence the contradiction with the assumption that the policy achieves $o(\log^2 T)$ regret under all settings. 
%
%Thus, we have that $\mathbb P(E_3) = 1 - \Omega(1)$. But now, under the original setting we have that $E[R] = \Omega(\log^2 T)$. Thus, the assumption that the policy achieves $o(\log^2 T)$ regret under all settings must be false. 


%\begin{align*}
%\mathbb P'(E_3) & = \mathbb E[ \mathbbm 1(E_3) e^{-\hat K_{t'}(\mu_b,\mu_b')}] \\ 
% &= \mathbb E[e^{-\hat K_{t'}(\mu_b,\mu_b')}] - o(E[e^{-\hat K_{t'}(\mu_b,\mu_b')}])  \\
%& \ge 
%\end{align*}



%\end{proof}










\subsection{Achieving Lower Bound via Balanced-Exploration}
\label{sec:waterfill}

%We saw above that being optimistic in the face of uncertainty and sampling at random achieve regret which is polynomial in the time horizon when the externality function is linear. 
We now present a policy which is cautious during the exploration phase, in that it pulls the arm with least accrued reward, to give it further opportunity to ramp up its score just in case its poor performance was bad luck. At the end of the exploration phase, it exploits the perceived best arm for the rest of the horizon.  

\begin{definition}
{\bf Balanced-Exploration($n$) Algorithm:} Fix $n\in \mathbb Z_+$.  
\begin{enumerate}
\item {\em Exploration phase:} Explore till (random) time $\tau_n$ where $\tau_n = \max(t:\exists b\in A s.t.\ S_b(t) < n)$, i.e., explore until each arm has incurred at least $n$ rewards. For $1\le t \le \tau_n$, pull arm $x(t) \in \arg\inf_{a \in A} S_a(t-1)$, with ties broken at random.
\item {\em Exploitation phase:} For $ \tau_n +1 \le t \le T$, pull the arm $\hat a^* \in \arg\inf_{a \in A} T_a(\tau_n)$, with ties broken at random.
\end{enumerate}
\end{definition}

%\virag{Can replace $\ceil{\ln^{1+\epsilon} T}$ with anything which is $\omega(\ln T)$.}

The following theorem provides a bound on the performance of the Balanced-Exploration($n$) policy. For the proof, see the Appendix.

\begin{theorem}\label{thm:Balanced-Exploration}
Suppose that $n = o(T)$. For each $\alpha$, there exists a constant $c_\alpha$ such that the regret under Balanced-Exploration($n$) policy satisfies the following: 
\begin{enumerate}
\item If $0< \alpha < 1$ then regret is $O(n^\alpha T^{1-\alpha}  + T e^{-c_\alpha n})$. Thus if $n = 2c_\alpha^{-1} \ln T$ then 
$$\mathbb E[R_T] = O(T^{1-\alpha}\ln^\alpha T).$$
\item If $\alpha = 1$ then regret is $O(n \ln T + T e^{-c_1 n}))$. Thus if $n = 2c_\alpha^{-1} \ln T$ then 
$$\mathbb E[R_T] = O(\ln^2 T).$$
\item If $\alpha >1$ then regret is $O(n^\alpha +  T e^{-c_\alpha n}))$. Thus if $n = 2c_\alpha^{-1} \ln T$ then 
$$\mathbb E[R_T] = O(\ln^\alpha T).$$
\end{enumerate}
\end{theorem}
Note that the constants $c_\alpha$ depend on the system parameters, namely, $\delta, \Delta, m,$ and $\alpha$ (but not on $(\mu_a)_{a\in A}$). This can be resolved by using $n$ as slightly larger than $O(\ln T)$ as noted below. 
\begin{corollary}
Fix a sequence $w_1,w_2,\ldots$ such that $w_k = \omega(1)$. For example, $w_k$ could be $\ln\ln k$ for each $k$. Set $n= w_T \ln T$. Then 
\begin{enumerate}
\item If $0< \alpha < 1$ then $\mathbb E[R_T] = O(w_T T^{1-\alpha}\ln^\alpha T)$.
\item If $\alpha = 1$ then $\mathbb E[R_T]  = O(w_T \ln^2 T)$.
\item If $\alpha >1$ then $\mathbb E[R_T]  = O(w_T\ln^\alpha T)$.
\end{enumerate}
\end{corollary}


%
%
%
%%$$ \mathbb P\left( \hat \mu_{a^*}(\tau)  < \hat \mu_b(\tau)\right)
%
%
%Let $E_n$ be event that $\sum_{k=1}^n \gamma_k >  2^{\alpha+1} n m/{\Delta}$. Then, \virag{Not really...also using the fact that there was more than certain number of samples.}
%
%\begin{multline}
%\mathbb P(\hat a^* \neq a^*) \le \mathbb P(\hat a^* \neq a^* | E_n^c) + \mathbb P(E_n) 
%			\le  e^{- c_1 n} + e^{-c_2 n}
%\end{multline}
%For some some constants $c_1$, $c_2$ which depend on system parameters. % $\mu_a$ for each $a$, $\Delta$, $m$, and $\alpha$ \virag{anything else they depend on?}. Thus, if $n = 2\max(1/c_1, 1/c_2)  \ln T)$ then $\mathbb P(\hat a^* \neq a^*)$ would be $O(1/T^2)$. However, $c_1,c_2$ depend on system parameters. Further, for the given $n$ the exploration time, i.e., $ 2^{\alpha+1} n m/{\Delta}$, depend on the system parameters. These issues get resolved if we set exploration time as $m^2 {\ln^{1+\epsilon} T}$, i.e., $\mathbb P(\hat a^* \neq a^*)$ is $O(1/T^2)$, without algorithm knowing the system parameters. 
%
%Thus, regret can be bounded as:
%
%\begin{multline} R \le m^2 \ceil{\ln^{1+\epsilon} T} +  \sum_{t= m^2 \ceil{\ln^{1+\epsilon} T} +1}^T \mathbb E \Big[ \frac{\sum_{a\neq a^*} f(N_a(t))}{\sum_{a} f(N_a(t))} \Big] \\+ T \; \mathbb P(\hat a^* \neq a^*),  
%\end{multline}
% where the first term accounts for exploration phase and the second term accounts for the expected number of times arm $a^*$ is not preferred during the exploitation phase. Note that, under $(\hat a^* \neq a^*)$, $\sum_{a\neq a^*} f(N_a(t))$ does not change after time $t= m^2 \ceil{\ln^{1+\epsilon} T}$. Further, by using argument similar to the above, w.h.p.\ we have that the total number of cycles during exploration phase, and thus the reward accrued by each arm in this phase, is $O( \ln^{1+\epsilon} T)$. 
% 
%Thus, we have 
%\begin{multline} R \le m^2 \ceil{\ln^{1+\epsilon} T}  \\ + O(m \ln^{1+\epsilon} T) \!\!\!\!\!\!\sum_{t= m^2 \ceil{\ln^{1+\epsilon} T} +1}^T \mathbb E \Big[ \frac{1}{\sum_{a} f(N_a(t))} \Big] + o(1)
%\end{multline}
%
%  Also, $ f(N_{a^*}(t)) \ge ....$...Need to argue this is close to $t$? 
%  
%    
%  For general rewards distributions, we can use convex ordering w.r.t. Bernoulli r.v.s. The $\max_a S_a(t)$ for each $t$ should be lower, and the $\min$ higher, and overall concentration should be better......
%
 
 % \begin{align*}
%  R \le m^2 \ceil{\ln^{1+\epsilon} T} + \sum_{t= m^2 \ceil{\ln^{1+\epsilon} T} +1}^T \frac{O( \ln^{1+\epsilon} T)}{O( \ln^{1+\epsilon} T) + t} + O(1/T),
% \end{align*}
% 
%\end{proof}









==> random.tex <==
% !TEX root = root.tex


\section{Random Explore-then-Exploit}
\label{sec:random}

%An intuition from previous section is that persistent positive bias towards the perceived best arm can be detrimental. In this section, we try the natural policy where each arm is chosen uniformly at random at all times, and thus has no such bias. 

%Since arms are chosen independently, one may as well assume that at each time an arm is selected first and then the preferences of the arrival are selected. Thus, both the preference models are statistically identical when Random policy is adopted. 

In this section, we consider an algorithm which chooses arms independently and uniformly at random for some period of time, and then commits to the empirical best arm for the rest of the time.  While such an algorithm explores all arms equally, it does not learn efficiently; in particular, it pulls suboptimal arms too frequently, and then has the risk of never recovering from the positive externalities generated by these arms (and the subsequent shifts in user population).   We formalize this intuition in this section.

To analyze this algorithm, we start with a technical result for the algorithm that {\em indefinitely} pulls arms independently and uniformly at random.  For the case where $f$ is linear, we can model the cumulative rewards obtained at each arm via the {\em generalized Friedman's urn process}.  These processes  are studied by embedding them into multitype continuous-time Markov branching processes \cite{AtK68,Jan04}, where the expected lifetime of each particle is one at all times. 

Here, we are interested in rewards obtained for more general $f$. We study this by considering multitype branching processes with state-dependent expected lifetimes. For technical reasons, we will assume that $\theta_a$ for each arm $a$ is integer valued and greater than or equal to $1$. This allows us to map our problem into an urn type process with initial number of balls of color $a$ in the urn being equal to $\theta_a$. We obtain the following result. For the proof, see the Appendix.

\begin{theorem}\label{thm:RandomAsymptotics}
Suppose that $\theta_a$ for each $a \in A$ is a positive integer. Suppose at each time step $t$ an arm is pulled independently and uniformly at random.
The following statements hold:
\begin{enumerate}[(i)]
\item If $f(x) = x^\alpha$ for $0<\alpha<1$ then for each $b \neq a^*$, we have that $\frac{N_{a^*}(t)}{N_b(t)} \to\frac{\theta_a}{\theta_b} \left(\frac{\mu_{a^*}}{\mu_{b}}\right)^{\frac{1}{1-\alpha}}$ almost surely as $t \to  \infty$. %Thus, Regret is $O(T)$. 
\item If $f(x) = x$ then for each $b \neq a^*$, we have that $\frac{N_{a^*}(t)}{(N_{b}(t))^\frac{\mu_{a^*}} {\mu_b}}$ converges  almost surely to a random variable $Y$ with $0<Y<\infty$ w.p. $1$. 
%\virag{Characterize $Y$ from Athreya and Karlin} %Thus, Regret is $O(T^\frac{\mu_{a'}}{\mu_{a^*}})$ where $a'$ is the arm with second largest expected reward. 
%\item  If $f(x) = \log x$, then the ratio involves Lambert W function, and we have linear regret......
\item If $f(x) = x^\alpha$ for $\alpha > 1$ then there is a positive probability that $N_{a^*}(t)$ is $O(1)$ while for some $b \neq a^*$ we have $N_b(t) \to \infty $ as $t \to \infty$.
\end{enumerate}
\end{theorem}

%\begin{proof} 
%\end{proof}

Clearly, by choosing arms at random at all times within time horizon the regret incurred is $\Theta(T)$. Thus, a natural policy is to select arms at random till time $\tau < T$ and pull the perceived best arm for the remaining time; this is what we mean by {\em random explore-then-exploit}. More formally:

\begin{definition}[Random($\tau$)]
Fix $\tau\in \mathbb Z_+$. Under Random($\tau$) policy, for each $1\le t\le \tau$, $I_t$ is chosen uniformly at random from set $A$. Let $\hat a^* \in \arg\max_a S_a(\tau)$, with tie broken at random. For $\tau <t < T$, $I_t = a^*$. 
\end{definition} 

Alternatively, one may choose $\hat a^* \in \arg\max_a  \frac{S_a(\tau)}{T_a(\tau)}$. The results below do not change due to exponential concentration in $T_a(\tau)$ w.r.t.\ $\tau$.  

In the light of Theorem~\ref{thm:RandomAsymptotics} one may envisage that for linear and sublinear $f$, Random($\tau)$ may perform well for some $\tau$. The following theorem provides performance bounds for the Random($\tau$) policy. For the proof, see the Appendix.

\begin{theorem}\label{thm:RandomRegret}
Suppose that $\theta_a$ for each $a \in A$ is a positive integer. Let $b = \arg \max_{a\neq{a^*}} \mu_a$. The following statements hold for Random($\tau$) policy for any $\tau$:
\begin{enumerate}[(i)]
\item If $0<\alpha<1$ then we have %$E[R] = \Omega(\tau^\alpha T^{1-\alpha} + T e^{-c \tau^{1-\alpha}}  )$ for some constant $c>0$. Optimizing over $\tau$, we obtain, 
$$\mathbb E[R_T] = \Omega(T^{1-\alpha} \ln^{\frac{\alpha}{1-\alpha}} T).$$ %Thus, Regret is $O(T)$. 
\item If $\alpha=1$ then we have %,at $\tau = T^{\frac{1}{1-\frac{\mu_{a^*}}{\mu_a}}}
$$\mathbb E[R_T] = \Omega\left(T^{\frac{\mu_b}{\mu_b+\theta_{a^*}\mu_{a^*}}}\right).$$
%
%\item  If $f(x) = \log x$, then the ratio involves Lambert W function, and we have linear regret......
\item If $\alpha > 1$ then we have 
$$\mathbb E[R_T] = \Omega(T) .$$
\end{enumerate}
\end{theorem}
%

Thus, for $\alpha > 1$, Random($\tau$) policy performs as poorly as UCB for any $\tau$. For $\alpha \le 1$, from Theorem~\ref{thm:RandomAsymptotics} we obtain that $\mathbb P(\hat a^* = a)$ tends to $1$ as $T,\tau \to \infty$. This is an improvement over the performance of UCB. Thus, a question arises, what is the optimal achievable regret performance when subjected to positive externalities? We address this question in the next section. 






==> ucb.tex <==
% !TEX root = root.tex

\section{Suboptimality of UCB algorithm}
\label{sec:ucb}

In this section we show that the standard UCB algorithm \cite{ACF02,Buc12}, which does not account for the positive externality, performs poorly. It is known that under the standard MAB setting the UCB($\gamma$) algorithm achieves $O(\ln T)$ regret when $\gamma > 2$.  For the standard Bernoulli MAB problem this is asymptotically optimal \cite{LaR85,Buc12}. Formally, the algorithm is defined as follows. 

\begin{definition}[UCB($\gamma$)]
Fix $\gamma > 0$. For each $a\in A$, let $\hat\mu_{a}(0) = 0$ and for each $t>0$ let $\hat\mu_{a}(t) \coloneqq \frac{S_{a}(t-1)}{T_{a}(t-1)}$, under convention that $\hat\mu_{a}(t) = 0$ if $T_{a}(t-1)=0$. For each $a\in A$ let $u_a(0) = 0$ and for each $t>0$ let 
$$u_a(t) \coloneqq  \hat\mu_{a}(t)+  \sqrt{\frac{\gamma \ln t}{T_a(t-1)}}. $$
Under UCB($\gamma$) policy, we have 
$$I_t \in \arg\max_{a\in A} u_a(t),$$
with ties broken uniformly at random. 
\end{definition}

Under our model, consider an event where $a^* \not\in J_t$ but $I_t = a^*$: i.e., $a^*$ is pulled but the arriving user did not prefer arm $a^*$.   Under UCB, such events are self-reinforcing, in that they not only lower the upper confidence bound for arm $a^*$, resulting in fewer future pulls of arm $a^*$, but they also reduce the preference of a {\em future users} towards arm $a^*$. In fact, the impact of this self-reinforcement under UCB is so severe that we obtain a striking result: there is a strictly positive probability that the optimal arm $a^*$ will {\em never} see a positive reward, as shown by the following theorem.  An immediate corollary of this result is that the regret of UCB is linear in the horizon length.  %For a proof of the theorem, see the Appendix.

\begin{theorem} \label{thm:UCB}
Suppose $\gamma > 0$. Suppose that $f(x)$ is $\Omega\left(\ln^{1+\epsilon}(x)\right)$ for some $\epsilon >0$. There exists an $\epsilon' > 0$ such that
$$\mathbb P\left(\lim_{T \to \infty} {S_{a^*}(T) =0} \right) \ge \epsilon'.$$ 
\end{theorem}

\begin{corollary}
The regret of UCB is $O(T)$. 
\end{corollary}


